Lower Ricci Curvature for Efficient Community Detection

This study introduces the Lower Ricci Curvature (LRC), a novel, scalable, and scale-free discrete curvature designed to enhance community detection in networks. Addressing the computational challenges posed by existing curvature-based methods, LRC offers a streamlined approach with linear computational complexity, making it well-suited for large-scale network analysis. We further develop an LRC-based preprocessing method that effectively augments popular community detection algorithms. Through comprehensive simulations and applications on real-world datasets, including the NCAA football league network, the DBLP collaboration network, the Amazon product co-purchasing network, and the YouTube social network, we demonstrate the efficacy of our method in significantly improving the performance of various community detection algorithms.

==> defs.tex <==
\usepackage[utf8]{inputenc}
\usepackage{geometry}
%\geometry{legalpaper, landscape, margin=2in}
%\geometry{legalpaper, margin=2in}
 \geometry{
 a4paper,
 total={170mm,257mm},
 left=20mm,
 top=20mm,
 }
\usepackage{amsmath,amssymb,graphicx,color,amsthm}
\usepackage[linesnumbered,ruled]{algorithm2e}
\usepackage{tikz}
\usepackage{dsfont}
\usepackage{mathtools}
\usetikzlibrary{shapes.geometric, arrows}
\usepackage{algorithmic}
%\usepackage{algpseudocode}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{mathrsfs}  
\usepackage{afterpage}
%\usepackage{subcaption,afterpage} 
\usepackage{mathtools}
%\usepackage{romannum}
\usepackage{amsfonts}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{enumerate}
\usepackage[round]{natbib}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{authblk}

%new math symbols taking no arguments
\newcommand{\parallelsum}{\mathbin{\!/\mkern-5mu/\!}}

\newcommand{\given}{\, |\,}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


\newcommand\<{\langle}
\newcommand\T{^\top}
\newcommand\CC{\mathbb{C}}
\newcommand\FF{\mathbb{F}}
\newcommand\NN{\mathbb{N}}
\newcommand\QQ{\mathbb{Q}}
\newcommand\RR{\mathbb{R}}
\newcommand\PP{\mathbb{P}}
\newcommand\ZZ{\mathbb{Z}}
\newcommand\EE{\mathbb{E}}
\newcommand\MM{\mathcal{M}}
\newcommand\WW{\mathcal{W}}
\newcommand\kk{\mathfrak{k}}
\newcommand\mm{\mathfrak{m}}
\newcommand\nn{\mathfrak{n}}
\newcommand\pp{\mathfrak{p}}
\newcommand\quq{\mathfrak{q}}
\newcommand\Gg{\mathfrak{g}}
\newcommand\GL{\mathrm{GL}}
\newcommand\SO{\mathrm{SO}}
\newcommand\Z{\widetilde{Z}}
\newcommand\from{\leftarrow}
\newcommand\into{\hookrightarrow}
\newcommand{\tr}{\operatorname{tr}}
\newcommand\onto{\twoheadrightarrow}
\newcommand\minus{\smallsetminus}
\newcommand\goesto{\rightsquigarrow}
\newcommand\dirlim{\varinjlim}
\newcommand\invlim{\varprojlim}
%redefined math symbols taking no arguments
\renewcommand\>{\rangle}
\renewcommand\iff{\Leftrightarrow}
\renewcommand\implies{\Rightarrow}
%\floatname{algorithm}{Procedure}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\bfx}{{X}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\vect}{\mathrm{Vec}}
\newcommand{\sg}{\Sigma}
\newcommand{\bfv}{{v}}
\newcommand{\bfc}{{c}}
\newcommand{\cnh}{\widehat{c}}
\newcommand{\hbfv}{\widehat{v}}
\newcommand{\vnh}{\widehat{V}}
\newcommand{\rnh}{\widehat{r}}
\newcommand{\PD}{\mathrm{PD}}
\newcommand{\eps}{\varepsilon}
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

%new math symbols taking arguments
\newcommand\ol[1]{{\overline{#1}}}

%redefined math symbols taking arguments
\renewcommand\mod[1]{\ (\mathrm{mod}\ #1)}
% Already in AOS template
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{example}{Example}
% \newtheorem*{example*}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
% \newtheorem{remark}{Remark}
% \newtheorem{note}{Note}
%math operators not in math italic font
\DeclareMathOperator\gr{gr}
\DeclareMathOperator\IN{\mathsf{in}}
\DeclareMathOperator\ass{Ass}
\DeclareMathOperator\GP{GP}
\DeclareMathOperator\tor{Tor}
\DeclareMathOperator\Ad{Ad}
\DeclareMathOperator\im{im}
\DeclareMathOperator\Sym{Sym}
\DeclareMathOperator\Hess{Hess}
\DeclareMathOperator\var{var}
\DeclareMathOperator\diag{diag}
\DeclareMathOperator\rees{\mathcal{R}}
\DeclareMathOperator\spec{Spec}
\DeclareMathOperator\length{length}
\DeclareMathOperator\argmin{argmin}
\DeclareMathOperator\argmax{argmax}
\DeclareMathOperator\ad{ad}
\DeclareMathOperator\Id{I}
\DeclareMathOperator\eig{eig}
\DeclareMathOperator\rank{rank}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
	#1\;\delimsize\|\;#2%
}
\newcommand{\KL}{KL\infdivx}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

%for easy 2 x 2 matrices
\newcommand\twobytwo[1]{\left[\begin{array}{@{}cc@{}}#1\end{array}\right]}

%for easy column vectors of size 2
\newcommand\tworow[1]{\left[\begin{array}{@{}c@{}}#1\end{array}\right]}

%for \marginpar to fit optimally
%hoffset=-1in
%\setlength\marginparwidth{2.2in}
%\setlength\marginparsep{1mm}


\newcommand\red[1]{\marginpar{\vspace{-1.4ex}\footnotesize{\color{red}#1}}}
\newcommand\score[1]{\marginpar{\colorbox{yellow}{#1/10}}}
\newcommand\total[1]{\marginpar{\colorbox{yellow}{\huge #1/100}}}
\newcommand\magenta[1]{\colorbox{magenta}{$\!$#1$\!$}}
\newcommand\yellow[1]{\colorbox{yellow}{$\!$#1$\!$}}
\newcommand\green[1]{\colorbox{green}{$\!$#1$\!$}}
\newcommand\cyan[1]{\colorbox{cyan}{$\!$#1$\!$}}
\newcommand\rmagenta[1]{\red{\magenta{\phantom{:}}\,: #1}}
\newcommand\ryellow[1]{\red{\yellow{\phantom{:}}\,: #1}}
\newcommand\rgreen[1]{\red{\green{\phantom{:}}\,: #1}}
\newcommand\rcyan[1]{\red{\cyan{\phantom{:}}\,: #1}}
\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}


\xdefinecolor{dukeblue}{rgb}{0.004,0.129,0.412}
\newcommand{\dl}[1]{\textcolor{dukeblue}{\textsf{DL: #1}}}
\newcommand{\ah}[1]{\textcolor{teal}{\textsf{AH: #1}}}
\newcommand{\indep}{\perp \!\!\! \perp}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
